A Temporal Anomaly Detection System for Vehicles utilizing Functional Working Groups and Sensor Channels

A modern vehicle fitted with sensors, actuators, and Electronic Control Units (ECUs) can be divided into several operational subsystems called Functional Working Groups (FWGs). Examples of these FWGs include the engine system, transmission, fuel system, brakes, etc. Each FWG has associated sensor-channels that gauge vehicular operating conditions. This data rich environment is conducive to the development of Predictive Maintenance (PdM) technologies. Undercutting various PdM technologies is the need for robust anomaly detection models that can identify events or observations which deviate significantly from the majority of the data and do not conform to a well defined notion of normal vehicular operational behavior. In this paper, we introduce the Vehicle Performance, Reliability, and Operations (VePRO) dataset and use it to create a multi-phased approach to anomaly detection. Utilizing Temporal Convolution Networks (TCN), our anomaly detection system can achieve 96% detection accuracy and accurately predicts 91% of true anomalies. The performance of our anomaly detection system improves when sensor channels from multiple FWGs are utilized.

==> table.tex <==
\begin{table*}
\centering
{
   % \rowcolors{1}{lightgray!20!}{}
   %\rowcolors{1}{cyan!20!}{}
   {\renewcommand{\arraystretch}{1.30}%
    \begin{tabularx}{\textwidth}{X|X|X|X|X|X}
   %\begin{tabularx}{p{0.2\textwidth}>{\centering}p{0.2\textwidth}>{\centering}p{0.2\textwidth}>{\centering}p{0.2\textwidth}>{\centering}p{0.2\textwidth}>{\centering\arraybackslash}p{0.2\textwidth}}
    \hline
    \rowcolor{lightgray!20!}
     \textbf{Subsystem} & 
    \textbf{Channel} & 
    \textbf{Unit} &
     \textbf{Range/Unit} & 
    \textbf{VIN 958 Range/Unit} & 
    \textbf{Description} &
    \hline
    
    
        
    \multirow{7}{*}{Engine}  & EngCoolantTemp             & Degree Fahrenheit \textit{(\degree F)}              & 190-230°F   & 21- 208             & Electric coolant fan activates when temp   exceeds 220° and turns off when it drops below 190°. \\\cline{2-6}
                              & PctEngLoad                 & Integer Percent, Percent Form & X           & 0-131               & Engine Load                                                                                     \\\cline{2-6}
                              & EngPctTorq                 & Integer Percent, Percent Form & X           & 0-131               & Engine Torque                                                                                   \\\cline{2-6}
                              & BoostPres                  & Pounds per Square Inch          & X           & 0-74                & X                                                                                               \\\cline{2-6}
                              & AccelPedalPos              & Integer Percent, Percent Form & X           & 0-99                & Accelerator Pedal Position                                                                        \\\cline{2-6}
                              & IntManfTemp                & Degree Fahrenheit  \textit{(\degree F)}            & X           & 23-176              & X                                                                                               \\\cline{2-6}
                              & EngRetarderStat\_1587      & Value                          & X           & 0-0                 & X                                                                                               \\\cline{2-6}
    \hline
    %==========================================%
    \multirow{8}{*}{Transmission} & VehSpeedEng                & Miles Per Hour (Mph)           & X           & 0-55                & Vehicle Speed                                                                                   \\\cline{2-6}
                              & TransOilTemp               & Degree Fahrenheit  \textit{(\degree F)}            & X           & 23-190              & Transmission Oil temperature                                                                  \\\cline{2-6}
                              & TrSelGr                    & Value                          & X           & -(127)    -- (+127) & Transmission Gear                                                                               \\\cline{2-6}
                              & TransDrivEng               & Value                          & X           & 3.0-3.0             & X                                                                                              \\\cline{2-6}
                              & TransTorqConv
                              LockupEngaged & Value                          & X           & 0 or 1              & Transmission Torque Converter   Status,                                                         \\\cline{2-6}
                              & TrOutShaftSp               & Revolution Per Minute (RPM)    & X           & 1--3243             & X                                                                                              \\\cline{2-6}
                              & ClutchSwtch                & Value                          &             & 0 or 3              & X                                                                                               \\\cline{2-6}
                              & TrShInProg                 & Value                          & X           & 3                   & X                                                                                               \\\cline{2-6}
        \hline
    %==========================================%
        \multirow{3}{*}{Fuel}         & FuelRate                   & Gallon (U.S) Per Hour (g/hr)   & X           & 0-18.7              & X                                                                                            \\\cline{2-6}
                              & InstFuelEco                & Gallon (U.S) Per Hour (g/hr)   & X           & 0-255.39            & X                                                                                               \\\cline{2-6}
                              & InjCtlPres                 & Pounds per Square Inch          & X           & 0 - 4060.8          & Injector Control Pressure                                                                       \\\cline{2-6}
    \hline
    %==========================================%
    
    Time                          & UTC\_1HZ                   & Seconds                        & Date-Time    & X                   & Timestamp                                                                                       \\
      \hline
    %==========================================%
Brake                         & BrakeSwitch                & Value                          & X           & 0                   & X                                                                                               \\
  \hline
    %==========================================%
Driveline                     & FrontAxleSpd               & Mile Per Hour (Mph)            & X           & 0-55                & X                                          \\
    %==========================================%   
    \hline
        \end{tabularx}
}
\caption{Description}
\label{table:features description}
}
\end{table*}
